Intrinsic timing properties of ideal 3D-trench silicon sensor with fast front-end electronics

This paper describes the fundamental timing properties of a single-pixel sensor for charged particle detection based on the 3D-trench silicon structure. We derive the results both analytically and numerically by considering a simple ideal sensor and the corresponding fast front-end electronics in two different case scenarios: ideal integrator and real fast electronics (trans-impedance amplifier). The particular shape of the Time of Arrival (TOA) distribution is examined and the relation between the time resolution and the spread of intrinsic charge collection time is discussed, by varying electronics parameters and discrimination thresholds. The results are obtained with and without simulated electronics noise. We show that the 3D-trench sensors are characterized by a $synchronous~region$, i.e. a portion of the active volume which leads to the same TOA values when charged particles cross it. The synchronous region size is dependent on the front-end electronics and discrimination threshold, and the phenomenon represents an intrinsic physical effect that leads to the excellent time resolution of these sensors. Moreover, we show that the TOA distribution is characterized by an intrinsic asymmetry, due to the 3D geometry only, that becomes negligible in case of significant electronics jitter.

==> bibl.tex <==
@INPROCEEDINGS{LaserIEEE,
  author={Aresti, Mauro and Brundu, Davide and Cardini, Alessandro and Contu, Andrea and Matteo Cossu, Gian and Dalla Betta, Gian-Franco and Garau, Michela and Lai, Adriano and Lampis, Andrea and Loi, Angelo},
  booktitle={2021 IEEE Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC)}, 
  title={A Complete in-Laboratory Characterization of 3D Trench-Type Silicon Pixel Sensors}, 
  year={2021},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/NSS/MIC44867.2021.9875786}
  }

@ARTICLE{Lai_review,
  
AUTHOR={Lai, Adriano},   
	 
TITLE={4D-tracking in the 10-ps range: A technological perspective},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={10},           
	
YEAR={2022},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fphy.2022.1019262},       
	
DOI={10.3389/fphy.2022.1019262},      
	
ISSN={2296-424X},   
   
ABSTRACT={The present paper focuses on recent and ready-to-come advancements concerning high-resolution 4D-tracking with a perspective approach. Four-dimensional-tracking techniques (particle tracking with timing information for each detection point) have revealed a necessity for the next and next-to-next generations of high-energy physics experiments to cope with the increasing luminosity and consequent event pile-up in the beam collision region. Such a decisive challenge concerns both detection and processing technologies at an unprecedented level of difficulty. In addition to the high performance required in space–time measurement precision (some tens of picoseconds resolution in timing and about 10 µm resolution in space), an extremely high radiation hardness is demanded for such technologies together with an extremely high read-out and processing capability. Emerging experimental solutions for sensors and electronics against such challenges are presented here.}
}

@article{CARTIGLIA2022167228,
title = {4D tracking: present status and perspectives},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {1040},
pages = {167228},
year = {2022},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2022.167228},
url = {https://www.sciencedirect.com/science/article/pii/S0168900222005824},
author = {N. Cartiglia and R. Arcidiacono and M. Costa and M. Ferrero and G. Gioachin and M. Mandurrino and L. Menzio and F. Siviero and V. Sola and M. Tornago}
}

@article{riegler,
    author = "Riegler, Werner and Aglieri Rinella, Gianluca",
    title = "{Time resolution of silicon pixel sensors}",
    eprint = "1706.04883",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    doi = "10.1088/1748-0221/12/11/P11017",
    journal = "JINST",
    volume = "12",
    number = "11",
    pages = "P11017",
    year = "2017"
}

@article{FastTiming,
    author = "Lai, Adriano and Cossu, Gian Matteo",
    title = "{High-resolution timing electronics for fast pixel sensors}",
    journal = "arXiv:2008.09867",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "Aug",
    year = "2020"
}

@article{FERNANDEZMARTINEZ201198,
title = {Simulation of new p-type strip detectors with trench to enhance the charge multiplication effect in the n-type electrodes},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {658},
number = {1},
pages = {98-102},
year = {2011},
note = {RESMDD 2010},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2011.04.056},
url = {https://www.sciencedirect.com/science/article/pii/S0168900211008400},
author = {P. Fernández-Martínez and G. Pellegrini and J.P. Balbuena and D. Quirion and S. Hidalgo and D. Flores and M. Lozano and G. Casse},
keywords = {p-type strip detectors, TCAD simulation}
}


@ARTICLE{tfboost_tcode,
AUTHOR={Brundu, D. and Contu, A. and Cossu, G. M. and Loi, A.},   
TITLE="{Modeling of Solid State Detectors Using Advanced Multi-Threading: The TCoDe and TFBoost Simulation Packages}",
JOURNAL={Frontiers in Physics},      
VOLUME={10},           
YEAR={2022},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2022.804752},       
DOI={10.3389/fphy.2022.804752},      
ISSN={2296-424X}
}


@article{Brundu_2021,
	doi = {10.1088/1748-0221/16/09/p09028},
	url = {https://doi.org/10.1088/1748-0221/16/09/p09028},
	year = 2021,
	month = {Sep},
	publisher = {{IOP} Publishing},
	volume = {16},
	number = {09},
	pages = {P09028},
	author = {D. Brundu and A. Cardini and A. Contu and G.M. Cossu and G.-F. Dalla Betta and M. Garau and A. Lai and A. Lampis and A. Loi and M.M. Obertino and B.G. Siddi and S. Vecchi},
	title = {Accurate modelling of 3D-trench silicon sensor with  enhanced timing performance and comparison with test beam measurements},
	journal = {Journal of Instrumentation},
}


@article{OptAbs,
  author={Green, M.A. and Keevers, M.J.},
  title="{Optical properties of intrinsic silicon at 300 K}", 
  journal={Progress in Photovoltaics: Research and Applications, Volume 3, Issue 3},
  year={1995},
  pages={189-192},
  doi={https://doi.org/10.1002/pip.4670030303},
  }

@article{NumDiff,
author = "{Michalcov\'a , V. and Kotrasov\'a, K. }", 
title = "{The Numerical Diffusion Effect on the CFD Simulation Accuracy of Velocity and Temperature Field for the Application of Sustainable Architecture Methodology}",
journal={Sustainability 2020, 12(23), 10173},
year ={2020, doi: https://doi.org/10.3390/su122310173},

}
@article{Medoncino,
title = "{3D trenched-electrode sensors for charged particle tracking and timing}",
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {927},
pages = {24-30},
year = {2019},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2019.02.015},
url = {https://www.sciencedirect.com/science/article/pii/S0168900219301901},
author = { Mendicino, R. and Forcolin, G. T. and Boscardin, M. and Ficorella, F. and Lai, A. and Loi, A. and Ronchin, S. and Vecchi, S. and {Dalla Betta}, G.-F. }
}


@article{JINST-TimeSpot,
author ={ Anderlini, L. and Aresti, M. and Bizzeti,A. and Boscardin, M. and Cardini, A. and Dalla Betta, G.-F. and Ferrero, M. and Forcolin, G. and Garau, M. and Lai, A. and Lampis, A. and Loi, A. and Lucarelli, C. and Mendicino, R. and Mulargia, R. and Obertino, M. and Robutti, E. and Ronchin, S. and Ruspa, M. and Vecchi, S.},
title ="{Intrinsic time resolution of 3D-trench silicon pixels for charged particle detection}", 
journal ={Journal of Instrumentation, 15, P09029},
year = {2020}
}

@article{Parker,
author ="{Parker, S.I. and Kok A., and Kenney C. and Jarron P. and Hasi J. and Despeisse M. and Da Via C. and Anelli G.}",
title = {Increased speed: 3D silicon sensors; Fast current ampliﬁers},
  journal={IEEE Trans. Nucl. Sci., 58 (2), pp. 404-417},
  year={2011}
}

@article{Ramo,
author = "{Ramo, S.}", 
title = "{Currents Induced by Electron Motion}",
journal={Proceedings of the IRE, vol. 27, no. 9, pp. 584-585},
year ={1939, doi: 10.1109/JRPROC.1939.228757},

}


@misc{TCode,
  author       = {Contu, A. and Loi, A.},
  title        = "{TimeSPOT COde for DEtector Simulation (TCoDe)}",
  year          = {2020, Zenodo, doi: 10.5281/zenodo.3686010},
  url          = {https://doi.org/10.5281/zenodo.3686010}
}
@misc{TCAD,
author = "{Synopsys Inc.}",
title  = "{Synopsys Sentaurus TCAD Version 2018.06 K-2015.06}", 
year = {2018},
url = {https://www.synopsys.com/silicon/tcad.html},
}

@article{FCC,
author = "{{FCC Collaboration}}",
title = "{The Future Circular Collider (FCC) Conceptual Design Report}", journal ={CERN-ACC-2018-0056, CERN-ACC-2018-0057, CERN-ACC-2018-0058, CERN-ACC-2018-0059},
year = {2018},
}
@article{CEPC,
author = {{CEPC Study Group}},
title ="{CEPC Conceptual Design Report}", 
journal ={arXiv:1809.00285},
year = {2018},
}

@incollection{Bosch,
title = "Chapter 21 - Deep Reactive Ion Etching",
editor = "Markku Tilli and Teruaki Motooka and Veli-Matti Airaksinen and Sami Franssila and Mervi Paulasto-Kröckel and Veikko Lindroos",
booktitle = "Handbook of Silicon Based MEMS Materials and Technologies (Second Edition)",
publisher = "William Andrew Publishing",
edition = "Second Edition",
address = "Boston",
pages = "444 - 469",
year = "2015",
series = "Micro and Nano Technologies",
isbn = "978-0-323-29965-7",
doi = "https://doi.org/10.1016/B978-0-323-29965-7.00021-X",
url = "http://www.sciencedirect.com/science/article/pii/B978032329965700021X",
author = "Franz Laermer and Sami Franssila and Lauri Sainiemi and Kai Kolari",
keywords = "Reactive ion etching, deep reactive ion etching, Bosch process, cryo-process, photoresist mask, notching effect, scalloping",
abstract = "This chapter discusses reactive ion etching and deep reactive ion etching on wafers detailing the various equipment and reactor requirements for different applications. The Bosch process is explained in detail as is cryogenic DRIE with details on the various etch masks for silicon. The issues and challenges of DRIE, such as vertical and sloped sidewalls, loading effect, lag, scalloping, notching effect are covered. This chapter also discusses the applications of DRIE such as free shape structures, small feature sizes, high aspect ratios, and deep and multidepth structures, as well as the post-DRIE etch treatments. The factors favoring either wet or dry etching are briefly given."
}





@article{CMS-TL,
author = "{{CMS Collaboration}}",
title ="{A MIP Timing Detector for the CMS Phase-2 Upgrade. Technical Design Report}", 
journal ={CERN-LHCC-2019-003, CMS-TDR-020},
year = {2019},
}
@article{ATLAS-TL,
author = "{{ATLAS Collaboration}}",
title = "{Technical Proposal: a High-Granularity Timing Detector for the ATLAS Phase-II Upgrade}", 
journal ={CERN-LHCC-2018-023, LHCC-P-012},
year = {2018},
}
@article{ufsdNONVA,
author = "{Mazza, {S.M}. and others}",
title = "{Properties of FBK UFSDs after neutron and proton irradiation up to $6\times 10^{15}$ ${\rm n}_{\rm eq}/{\rm cm}^2$}", 
journal ={arXiv:1804.05449v3},
year = {2018},
}
@article{ufsd,
    title={Proprieties of FBK UFSDs after neutron and proton irradiation up to 6*10e15 neq/cm2},
    author={Mazza, {S.M}. and others},
    year={2018},
    eprint={1804.05449},
    journal ={arXiv:1804.05449v3},
    archivePrefix={arXiv},
    primaryClass={physics.ins-det}
}
@article{3D,
author = "Parker, S. and others",
title = "3D - A proposed new architecture for solid-state radiation detectors",
journal ={NIM A395, 328-34},
year = {1997}
}

@article{pps,
author = "{{CMS Collaboration}}",
title = "{The PPS tracking system: performance in LHC Run2 and prospects for LHC Run3}",
journal = "JINST",
volume= "15",
year  = "2020, doi: 10.1088/1748-0221/15/05/C05049",
pages = "C05049",
}

@article{ibl,
author = "Abbot, B. and others,",
title = "{Production and integration of the ATLAS Insertable B-Layer}",
journal = "JINST",
volume  = "13",
year    = "2018, doi: 10.1088/1748-0221/13/05/t05008",
pages = "T05008",
}

@article{3Dradhard,
	doi = {10.1088/1748-0221/13/09/p09009},
	url = {https://doi.org/10.1088/1748-0221/13/09/p09009},
	year = 2018,
	publisher = {{IOP} Publishing},
	volume = {13},
	number = {09},
	pages = {P09009},
	author = {J. Lange and G. Giannini and S. Grinstein and M. Manna and G. Pellegrini and D. Quirion and S. Terzo and D. V{\'{a}}zquez Furelos},
	title = {Radiation hardness of small-pitch 3D pixel sensors up to a fluence of $3 \times 10^{16}$ ${\rm n}_{\rm eq}/{\rm cm}^2$},
	journal = {Journal of Instrumentation},
}

@misc{quartz,
note = {Helios Italquartz, quarz type NHI-1200}
}

@misc{optical-silicon,
note = "Wacker,  crystal clear elastomer ELASTOSIL RT601",
url = "https://www.wacker.com/h/en-it/c/elastosil-rt-601-ab/p/000005741"
}

@misc{planacon,
note = {Photonis Netherland B.V., Planacon micro-channel plate photomultiplier model XP85012 and XP85112},
url = "https://www.photonis.com/products/planacon",
}

@misc{oscilloscope,
note = {Rohde \& Schwarz, digital oscilloscope RTP084},
url = "https://www.rohde-schwarz.com/product/rtp-productstartpage_63493-469056.html",
}
%
@misc{llcable,
note = {Siretta Ltd., low loss 50 Ohms coaxial cable type LLC200A, p/n ASME1000F058L13},
}
%%,
      
@article{HiLumiLHCNONVA,
      author        = "{Apollinari, G. and Béjar Alonso, I. and Brüning, O. and  Lamont, M. and Rossi, L.}",
      title         = "High-Luminosity Large Hadron Collider (HL-LHC):
                       Preliminary Design Report",
      publisher     = "CERN",
      address       = "Geneva",
      journal        = "CERN Yellow Reports: Monographs",
      year          = "2015, doi: 10.5170/CERN-2015-005",
      url           = "https://cds.cern.ch/record/2116337"
}
@article{HiLumiLHC,
      author        = "{Apollinari, G. and others}",
      title         = "High-Luminosity Large Hadron Collider {(HL-LHC)}:
                       Preliminary Design Report",
      publisher     = "CERN",
      address       = "Geneva",
      journal        = "CERN Yellow Reports: Monographs",
      year          = "2015, doi: 10.5170/CERN-2015-005",
      url           = "https://cds.cern.ch/record/2116337"
}
@article{LHCb-PII-Physics,
      title         = "{Physics case for an LHCb Upgrade II --- Opportunities in flavour physics, and beyond, in the HL-LHC era}",
      institution   = "CERN",
      author = "{{LHCb collaboration}}",
      address       = "Geneva",
      journal       = "CERN-LHCC-2018-027, LHCb-PUB-2018-009",
      year          = "2018",
      eprint         = "1808.08865",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
}

@article{LHCb-PII-EoI,
      title         = "{Expression of Interest for a Phase-II LHCb Upgrade:
                       Opportunities in flavour physics, and beyond, in the HL-LHC
                       era}",
      institution   = "CERN",
      author = "{{LHCb collaboration}}",
      address       = "Geneva",
      journal       = "CERN-LHCC-2017-003",
      year          = "2017",
}
@article{Vertex,
author = "Lai, A.",
title  = "{Recent results of the TIMESPOT project on sensors and electronics developments for future vertex detectors}",
journal = "{Talk given at "28th International Workshop on Vertex Detectors (VERTEX)", Lopud Island, Croatia, October 13-18, 2019}",
volume = "VERTEX2019",
year  = "2019, doi: 10.22323/1.367.0029"
}
@article{ForcolinIEEE,
author = "Forcolin, G. and others",
title = "Development of 3D Trenched-Electrode Pixel Sensors with Improved Timing performance",
journal =  "{Proceedings IEEE NSS Conference, October 2019}",
year  = "2019"
}
@article{ForcolinJINST,
author = "Forcolin, G. and others",
title = "Development of 3D Trenched-Electrode Pixel Sensors with Improved Timing performance",
journal = "JINST",
volume  = "14",
year    = "2019",
pages = "C07011"
}
@article{Siena,
author = "Mulargia, R. and others",
title = "Tracking with timing: the TIMESPOT project",
journal  = {Proceedings of the "15th Topical Seminar on Innovative Particle and Radiation Detectors (IPRD19)",  Siena, Italy, October 14-17, 2019, to appear in JINST},
year  = "2019",
}

@article{PELLEGRINI201412,
title = {Technology developments and first measurements of Low Gain Avalanche Detectors (LGAD) for high energy physics applications},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {765},
pages = {12-16},
year = {2014},
note = {HSTD-9 2013 - Proceedings of the 9th International "Hiroshima" Symposium on Development and Application of Semiconductor Tracking Detectors},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2014.06.008},
url = {https://www.sciencedirect.com/science/article/pii/S0168900214007128},
author = {G. Pellegrini and P. Fernández-Martínez and M. Baselga and C. Fleta and D. Flores and V Greco and S. Hidalgo and I. Mandić and G. Kramberger and D. Quirion and M. Ullan},
keywords = {Silicon detectors, Avalanche multiplication, Radiation hardness},
abstract = {This paper introduces a new concept of silicon radiation detector with intrinsic multiplication of the charge, called Low Gain Avalanche Detector (LGAD). These new devices are based on the standard Avalanche Photo Diodes (APD) normally used for optical and X-ray detection applications. The main differences to standard APD detectors are the low gain requested to detect high energy charged particles, and the possibility to have fine segmentation pitches: this allows fabrication of microstrip or pixel devices which do not suffer from the limitations normally found [1] in avalanche detectors. In addition, a moderate multiplication value will allow the fabrication of thinner devices with the same output signal of standard thick substrates. The investigation of these detectors provides important indications on the ability of such modified electrode geometry to control and optimize the charge multiplication effect, in order to fully recover the collection efficiency of heavily irradiated silicon detectors, at reasonable bias voltage, compatible with the voltage feed limitation of the CERN High Luminosity Large Hadron Collider (HL-LHC) experiments [2]. For instance, the inner most pixel detector layers of the ATLAS tracker will be exposed to fluences up to 2×10161MeVneq/cm2, while for the inner strip detector region fluences of 1×1015neq/cm2 are expected. The gain implemented in the non-irradiated devices must retain some effect also after irradiation, with a higher multiplication factor with respect to standard structures, in order to be used in harsh environments such those expected at collider experiments.}
}

@article{Hiroshima,
title = "First results of the {TIMESPOT} project on developments on fast sensors for future vertex detectors",
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {981},
pages = {164491},
year = {2020},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2020.164491},
url = {https://www.sciencedirect.com/science/article/pii/S0168900220308883},
author = {A. Lai and L. Anderlini and M. Aresti and A. Bizzeti and A. Cardini and G.-F. Dalla Betta and G.T. Forcolin and M. Garau and A. Lampis and A. Loi and C. Lucarelli and R. Mendicino and R. Mulargia and M. Obertino and E. Robutti and S. Vecchi}
}

@phdthesis{PhD_ALoi,
author = "Loi, A.",
title = "Design and test of a timing optimized {3D} silicon sensor for HL-LHC experiments",
journal = "PhD Thesis, 4-feb-2020", 
url= {http://hdl.handle.net/11584/284136},
year = {2020},
type     = {{PhD} dissertation},
school = "{Univestit\`a di Cagliari, Italy}"
}

@article{Geant4,
     author    = "Agostinelli, S. and others", 
     collaboration = "{{Geant4 collaboration}}",
     title     = "{Geant4: A simulation toolkit}",
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {506},
number = {3},
pages = {250-303},
     year      = {2003},
doi={10.1016/S0168-9002(03)01368-8}
}

@article{Geant4_b,
      author         = "Allison, J. and others", 
      collaboration  = "{{Geant4 collaboration}}",
      title          = "{Geant4 developments and applications}",
      journal        = "IEEE Trans. Nucl. Sci.",
      volume         = "53",
      pages          = "270",
      year           = "2006, doi: 10.1109/TNS.2006.869826",
      reportNumber   = "SLAC-PUB-11870",
}

@article{Meroli_Landau,
author = {Meroli, S. and Passeri, D. and Servoli, L.},
title = "{Energy loss measurement for charged particles in very thin silicon layers}",
year = {2011, doi: 10.1088/1748-0221/6/06/P06013},
month = {06},
pages = {P06013},
volume = {6},
journal = {Journal of Instrumentation},
}%[http://meroli.web.cern.ch/Lecture\_StragglingFunction.html]

@article{FastTiming,
      title={High-resolution timing electronics for fast pixel sensors}, 
      author={Lai A. and Cossu G. M.},
      year={2020, arXiv:2008.09867},
      eprint={2008.09867},
      archivePrefix={arXiv},
      primaryClass={physics.ins-det}
}   

@article{GOULDING1966,
title = {Semiconductor detectors for nuclear spectrometry, I},
journal = {Nuclear Instruments and Methods},
volume = {43},
number = {1},
pages = {1-54},
year = {1966},
note = {Proceedings of the Tenth Summer Meeting of Nuclear Physicists},
issn = {0029-554X},
doi = {https://doi.org/10.1016/0029-554X(66)90531-3},
url = {https://www.sciencedirect.com/science/article/pii/0029554X66905313},
author = {F.S Goulding},
abstract = {These papers were prepared primarily as background information for attendees at the meeting who have not been directly concerned with the development of detectors. The first chapter contains information on semi-conductor materials and the theory of junctions necessary for an understanding of detectors. In the second chapter the methods of making detectors by diffusion and also by lithium drifting are detailed and the relative merits of different types of detectors are discussed. We then consider the problems associated with obtaining good energy resolution in detector systems dealing primarily with electrical noise and statistical fluctuations of the charge produced in the detector. In the final chapter, a semi-theoretical treatment of the detector pulse shape considerations is given and the subject of radiation damage is discussed. While the treatment is generally applicable to detector systems the author has made no effort to write a review of the voluminous literature on this subject. The methods of detector manufacture, for example, are representative of only a portion of our own group's work in this area and are only to be regarded as indicative of a general technique. Other papers presented at the conference describe methods used by other groups.}
}
      
@article{UCSC,
author = {UcscSingleChannel},
title = "twiki.cern.ch/twiki/bin/view/Main/UcscSingleChannel"
      }

@article{RiassuntoEUStrat,
author = {Aleksa, M. and others},
title = "Strategic {RD} Programme on Technologies for Future Experiments", 
journal ="Tech. Rep. CERN-OPEN-2018-006, CERN, Geneva",
year ={2018},
url = "https://cds.cern.ch/record/2649646"
}
@article{nINp,
author = {Lozano, M. and others},
title = "Comparison of radiation hardness of {P-in-N}, N-in-N, and N-in-P silicon pad detectors",
journal = {IEEE Transactions on Nuclear Science},  
year={2005},  
volume={52},  
number={5},  
pages={1468-1473}
}

@article{TFBoost_cit,
  author       = {Brundu, D. and Cossu, G. M.},
  title        = "dbrundu/{TFBoost: TFBoost} v0.2-alpha",
  month        = nov,
  year         = {2020, Zenodo. doi: 10.5281/zenodo.4291148},
  publisher    = {Zenodo},
  version      = {v0.2-alpha},
  doi          = {10.5281/zenodo.4291148},
  url          = {https://doi.org/10.5281/zenodo.4291148}
}

@article{SCHARF20151,
title = {Determination of the electronics transfer function for current transient measurements},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {779},
pages = {1-5},
year = {2015},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2014.12.016},
url = {https://www.sciencedirect.com/science/article/pii/S0168900214014570},
author = {C. Scharf and R. Klanner}
}

@article{deconv_problem,
  author={S. M. {Riad}},
  journal={Proceedings of the IEEE}, 
  title={The deconvolution problem: An overview}, 
  year={1986},
  volume={74},
  number={1},
  pages={82-85},
  doi={10.1109/PROC.1986.13407}}
  
@MISC{deconv_noise,
       author = {{Nahman}, N.~S. and {Guillaume}, M.~E.},
        title = "{Deconvolution of time domain waveforms in the presence of noise}",
     keywords = {Convolution Integrals, Noise (Sound), Time Functions, Waveforms, Broadband, Coaxial Cables, Dynamic Response, Radio Antennas, Signal To Noise Ratios, Signal Transmission, Wave Propagation, Electronics and Electrical Engineering},
 howpublished = {NASA STI/Recon Technical Report N},
         year = {1981, https://ui.adsabs.harvard.edu/abs/1981STIN...8227682N},
        month = oct,
        pages = {27682},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981STIN...8227682N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{red_noise_lect,
  author        = {Hartmann, D. L.},
  title         = "Objective Analysis, course notes, https://atmos.uw.edu/$\sim$dennis/552\_{Notes}\_ftp.html, chapter 6a",
  month         = {February},
  year          = {2013 },
  publisher={Department of Atmospheric sciences, University of Washington}
}

@misc{hydra,
  author       = {Alves Junior, A. A.},
  title        = {MultithreadCorner/Hydra},
  year         = {2018, Zenodo,  doi: 10.5281/zenodo.1206261},
  url          = {https://doi.org/10.5281/zenodo.1206261}
}

@article{hydra2,
    author = "Alves Jr, A. A. and Sokoloff, M. D.",
    title = "{Hydra: a C++11 framework for data analysis in massively parallel platforms}",
    eprint = "1711.05683",
    archivePrefix = "arXiv",
    primaryClass = "cs.MS",
    doi = "10.1088/1742-6596/1085/4/042013",
    journal = "J. Phys. Conf. Ser.",
    volume = "1085",
    number = "4",
    pages = "042013",
    year = "2018"
}

@incollection{lambert,
author = {Lambert, J.~H.},
title  = {Photometria sive de mensura et gradibus luminis, colorum et umbrae},
year   = {1760},
publisher = {Detleffsen},
address = {Augusta}
}

@ARTICLE{beer,
author = {Beer, A},
title = {Bestimmung der Absorption des rothen Lichts in farbigen Flüssigkeiten}, journal ={Annalen der Physik und Chemie}, 
volume = {86},
year = {1852}, 
pages = {78-88}
}

@article{ARCmethod,
title = "Comparative study of the timing techniques currently employed with {Ge} detectors",
journal = {Nuclear Instruments and Methods},
volume = {98},
number = {2},
pages = {335-347},
year = {1972},
issn = {0029-554X},
doi = {https://doi.org/10.1016/0029-554X(72)90115-2},
url = {https://www.sciencedirect.com/science/article/pii/0029554X72901152},
author = {Z.H. Cho and R.L. Chase},
}


@article{directBond,
author = {Shimbo,M.  and Furukawa,K.  and Fukuda,K.  and Tanzawa,K. },
title = {Silicon‐to‐silicon direct bonding method},
journal = {Journal of Applied Physics},
volume = {60},
number = {8},
pages = {2987-2989},
year = {1986},
doi = {10.1063/1.337750},
URL = {https://doi.org/10.1063/1.337750},
eprint = {https://doi.org/10.1063/1.337750}
}


@article{Andreatrento,
      author        = "Lampis, A.",
      title         = "{Sub-pixel characterization of innovative 3D trench-design silicon pixel sensors using ultra-fast laser-based testing equipment}",
      month         = "Feb",
      year          = "2021,  https://indico.cern.ch/event/983068/contributions/4223202/",
      journal = "16th Trento Workshop on Advanced Silicon Radiation Detectors"
}

@misc{IRlaser,
note = "NTK Photonics, OneFive Origami 10-40,https://www.nktphotonics.com/lasers-fibers/product/onefive-origami-ultra-low-noise-femtosecond-laser/"
}


@article{Allpix2,
    author = {Spannagel, S. and Wolters, K. and Hynds, D. and Alipour Tehrani, N. and Benoit, M. and Dannheim, D. and Gauvin, N. and N\"urnberg, A. and Sch\"utze, P. and Vicente Barreto Pinto, M.},
    title = "{Allpix$^2$: A Modular Simulation Framework for Silicon Detectors}",
    eprint = "1806.05813",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CLICdp-Pub-2018-002, CLICDP-PUB-2018-002",
    doi = "10.1016/j.nima.2018.06.020",
    journal = "Nucl. Instrum. Meth. A",
    volume = "901",
    pages = "164--172",
    year = "2018"
}


@misc{kdetsim,
note = "G. Kramberger,  KDetSim - a simple way to simulate detectors, http://kdetsim.org/"
}

@misc{wgtfield2,
note = "N. Cartiglia et al.,  Weightfield2:  a freeware 2D simulator for silicon and diamond detector, http://personalpages.to.infn.it/~cartigli/Weightfield2/Main.html"
}

@book{Razavi,
author = {Razavi, B.},
title = {Design of Integrated Circuits for Optical Communications},
year = {2002},
isbn = {0072822589},
publisher = {McGraw-Hill, Inc.},
address = {USA},
edition = {1}
}


@Misc{riegler_ppt,
author = {{Werner Riegler}},
title = "{Time resolution of silicon sensors}",
howpublished = {CERN Detector Seminar, \textsc{url:}~\url{https://indico.cern.ch/event/1083146/attachments/2328724/3975380/detector_seminar_oct_15_2021_timing_riegler_v2.pdf}},
year = {2021}
}

@article{Ramo,
author = "{Ramo, S.}", 
title = "{Currents Induced by Electron Motion}",
journal={Proceedings of the IRE, vol. 27, no. 9, pp. 584-585},
year ={1939, doi: 10.1109/JRPROC.1939.228757}
}

@article{Lampis:2022lpj,
doi = {10.1088/1748-0221/18/01/C01051},
url = {https://dx.doi.org/10.1088/1748-0221/18/01/C01051},
year = {2023},
month = {jan},
publisher = {IOP Publishing},
volume = {18},
number = {01},
pages = {C01051},
author = {A. Lampis and F. Borgato and D. Brundu and A. Cardini and G.M. Cossu and G.-F. Dalla Betta and M. Garau and L. La Delfa and A. Lai and A. Loi and M. Obertino and G. Simi and S. Vecchi},
title = {10 ps timing with highly irradiated 3D trench silicon pixel sensors},
journal = {Journal of Instrumentation},
abstract = {In this paper the results of a beam test characterization campaign of 3D trench silicon pixel sensors are presented. A time resolution in the order of 10 ps was measured both for non-irradiated and irradiated sensors up to a fluence of 2.5 × 1016 1 MeV neq cm−2. This feature and a detection efficiency close to 99% make this sensors one of the best candidates for 4D tracking detectors in High-Energy-Physics experiments.}
}

@ARTICLE{Testbeam10ps,
  
AUTHOR={Borgato, F. and Brundu, D. and Cardini, A. and Cossu, G. M. and Dalla Betta, G. F. and Garau, M. and La Delfa, L. and Lai, A. and Lampis, A. and Loi, A. and Obertino, M. M. and Simi, G. and Vecchi, S.},   
	 
TITLE={Charged-particle timing with 10 ps accuracy using TimeSPOT 3D trench-type silicon pixels},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={11},           
	
YEAR={2023},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fphy.2023.1117575},       
	
DOI={10.3389/fphy.2023.1117575},      
	
ISSN={2296-424X}

}

@article{FastTiming,
      title={High-resolution timing electronics for fast pixel sensors}, 
      author={Lai A. and Cossu G. M.},
      year={2020, arXiv:2008.09867},
      eprint={2008.09867},
      archivePrefix={arXiv},
      primaryClass={physics.ins-det}
}   
